Keep Your Transactions On Short Leashes

The adversary's goal in mounting Long Range Attacks (LRAs) is to fool potential victims into using and relying on a side chain, i.e., a false, alternate history of transactions, and into proposing transactions that end up harming themselves or others. Previous research work on LRAs on blockchain systems have used, at a high level, one of two approaches. They either try to (1) prevent the creation of a bogus side chain or (2) make it possible to distinguish such a side chain from the main consensus chain. In this paper, we take a different approach. We start with the indistinguishability of side chains from the consensus chain -- for the eclipsed victim -- as a given and assume the potential victim will be fooled. Instead, we protect the victim via harm reduction applying "short leashes" to transactions. The leashes prevent transactions from being used in the wrong context. The primary contribution of this paper is the design and analysis of leashes. A secondary contribution is the careful explication of the LRA threat model in the context of BAR fault tolerance, and using it to analyze related work to identify their limitations.

==> author-acm.tex <==
%\authorinfo{
%{\rm
%  Raymond Cheng$^{\dag}$,
%}\\
%{\small
%  $\dag$University of Washington
%}
%}

\fancyhf{} % Remove fancy page headers 
\fancyhead[C]{Anonymous submission \#103 to ACM CCS 2017}
\fancyfoot[C]{\thepage}

\setcopyright{none} % No copyright notice required for submissions
\acmConference[Anonymous Submission to ACM CCS 2017]{ACM Conference on Computer and Communications Security}{Due 19 May 2017}{Dallas, Texas}
\acmYear{2017}

% TODO: replace this section with code generated by the tool at https://dl.acm.org/ccs.cfm
\begin{CCSXML}
  <ccs2012>
  <concept>
  <concept_id>10002978.10002991.10002994</concept_id>concept_id>
  <concept_desc>Security and privacy~Pseudonymity, anonymity and untraceability</concept_desc>concept_desc>
  <concept_significance>500</concept_significance>concept_significance>
  </concept>concept>
  <concept>
  <concept_id>10002978.10002991.10002995</concept_id>concept_id>
  <concept_desc>Security and privacy~Privacy-preserving protocols</concept_desc>concept_desc>
  <concept_significance>500</concept_significance>concept_significance>
  </concept>concept>
  </ccs2012>ccs2012>
\end{CCSXML}

\ccsdesc[500]{Security and privacy~Pseudonymity, anonymity and untraceability}
\ccsdesc[500]{Security and privacy~Privacy-preserving protocols}
% -- end of section to replace with generated code

\keywords{privacy, anonymity, messaging} % TODO: replace with your keywords


==> author-ieee.tex <==
%\author{\rm Paper \#50}
\author{
  \IEEEauthorblockN{Raymond Cheng\IEEEauthorrefmark{1}, xxx\IEEEauthorrefmark{2}}
  \IEEEauthorblockA{\IEEEauthorrefmark{1}UC Berkeley
  \\\{ryscheng, xxx\}@cs.berkeley.edu}
  \IEEEauthorblockA{\IEEEauthorrefmark{2}YYY
  \\yyy@uw.edu}
}


==> main.tex <==
\newif\ifOverleaf
\Overleaftrue
\input{paper-docclass}
\input{paper-common}


==> paper-docclass.tex <==
% style/head-* files has \documentclass but arxiv looks for it, so the
% entry points paper.tex for normal use, main.tex for overleaf, and
% arxiv.tex for arxiv's autotex to recognize and use need this
% separated out.

%\input{style/head-acm}
%\input{style/head-ieee}
%\input{style/head-usenix} % usenix style has no date
\input{style/head-plain}
%\input{style/head-plain-1col}


==> paper.tex <==
\newif\ifOverleaf
\Overleaffalse
\input{paper-docclass}
\input{paper-common}

